Recent Improvements for the Lepton Propagator PROPOSAL

The lepton propagator PROPOSAL is a Monte-Carlo Simulation library written in C++, propagating high energy muons and other charged particles through large distances of media. In this article, a restructuring of the code is described, which yields a performance improvement of up to $30\,\%$. For an improved accuracy of the propagation processes, more exact calculations of the leptonic and hadronic decay process and more precise parametrizations for the interaction cross sections are now available. The new modular structure allows a more flexible and custom usage, which is further facilitated with a python interface.

==> Makefile <==
all: build/article.pdf

build/article.pdf: FORCE
	latexmk \
	 --pdf \
	 --output-directory=build \
	 --halt-on-error \
	 --interaction=nonstopmode \
	 article.tex

FORCE:

clean:
	rm -rf build

.PHONY: all clean FORCE

